Motion Planning Transformers: A Motion Planning Framework for Mobile Robots

Fast and efficient sampling-based motion planning (SMP) is an integral component of many robotic systems, such as autonomous cars. A popular technique to improve the efficiency of these planners is to restrict search space in the planning domain. Existing algorithms define parametric functions to bound the search space, but these do not extend to non-holonomic robotic systems. Recent learning-based methods use a combination of convolutional and fully connected networks to encode the planning space. However, these methods are restricted to fixed map sizes, which are often not realistic in the real world. In this paper, we introduce a transformer-based approach, Motion Planning Transformer, to restrict the search space by learning to discern regions with a valid path from prior data. The model learns not only to restrict search spaces for simple 2D systems but also for non-holonomic robotic systems. We validate our method on various randomly generated environments with different map sizes and plan trajectories for a physical non-holonomic robot. We also provide a ROS2 plugin of our method for the Nav2 planning stack. The results show that our method reduces search space nodes by 2-12 times compared to traditional planners and has better generalizability than recent learning-based planners.

==> 5.5Discussions.tex <==
Graph-based search methods such as A* can also be used to solve the given planning problem using the costmap, but in order to do real time planning, these methods often require sub-sampling of the costmap to provide solutions in real time. Further hand-tuned heuristics are required to restrict the planning space for kinematically constrained systems \cite{doi:10.1177/0278364909359210} otherwise they get stuck in local minima \cite{doi:10.1177/02783640122067453}. We have shown through our experiments that the MPT aided planners require no such sub-sampling, and can learn to restrict search spaces by leveraging data. Since MPT is agnostic to the underlying planner, graph-based searches can also be used to search the highlighted space. 

Prior learning-based methods that predict a value such as VIN \cite{tamar2016value} are difficult to train for larger maps \cite{nardelli2018value} because of the depth of layers required to propagate the reward. Other learning-based planners, such as Neural Exploration-Exploitation Tree (NEXT) \cite{DBLP:conf/iclr/ChenDLYLS20}, get stuck in local minimums resulting in longer search times and reduced accuracy (see Supplementary Materials Section B). The transformer-based planner proposed by \cite{chaplot2021differentiable} uses fixed encoding, resulting in its ability to generalize to maps of larger sizes. Moreover, map sizes used in our experiments are nearly ten times larger than those in [5]. Moreover, MPT combines the best of both worlds by learning from data the space where a plan exists and using an optimal planner to get the exact path.
